DELIFT: Data Efficient Language model Instruction Fine Tuning

Fine-tuning large language models (LLMs) is essential for enhancing their performance on specific tasks but is often resource-intensive due to redundant or uninformative data. To address this inefficiency, we introduce DELIFT (Data Efficient Language model Instruction Fine-Tuning), a novel algorithm that systematically optimizes data selection across the three key stages of fine-tuning: (1) instruction tuning, (2) task-specific fine-tuning (e.g., reasoning, question-answering), and (3) continual fine-tuning (e.g., incorporating new data versions). Unlike existing methods that focus on single-stage optimization or rely on computationally intensive gradient calculations, DELIFT operates efficiently across all stages. Central to our approach is a pairwise utility metric that quantifies how beneficial a data sample is for improving the model's responses to other samples, effectively measuring the informational value relative to the model's current capabilities. By leveraging different submodular functions applied to this metric, DELIFT selects diverse and optimal subsets that are useful across all stages of fine-tuning. Experiments across various tasks and model scales demonstrate that DELIFT can reduce the fine-tuning data size by up to 70% without compromising performance, offering significant computational savings and outperforming existing methods in both efficiency and efficacy.

==> name.tex <==
data point1 : how are you

data point 2: how is the weekend

[p1] [p2] -> similarity

costs in time (breakdown of costs, inference/training)

------
|     |
|     |
-----

==> tables/benchmark.tex <==
% \begin{table}[]
% \centering
% \begin{tabular}{c|cc|cc}
% \hline
% Method        & \multicolumn{2}{c|}{Phi-3} & \multicolumn{2}{c}{Qwen2} \\ \hline
%               & ICL            & QLoRA          & ICL           & QLoRA         \\ \hline
% Initial       &                &                &               &               \\
% Random        &                &                &               &               \\
% SelectIT      &                &                &               &               \\
% LESS          &                &                &               &               \\
% Sem Sim Util. &                &                &               &               \\
% ICL Util      & {\ul }         & \textbf{}      & {\ul }        & {\ul }        \\
% Full Data     & \textbf{}      & {\ul }         & \textbf{}     & \textbf{}     \\ \hline
% \end{tabular}
% \caption{Classification accuracy (\%) on Qwen2 and Phi-3 on HotpotQA and MMLU.}
% \label{uc2: qwen-phi-hotpot-mmlu}
% \end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{c|ccc|ccc}
% \hline
% Method        & \multicolumn{3}{c|}{ICL} & \multicolumn{3}{c}{QLoRA} \\ \hline
%               & ROUGE  & BGE  & LLM-A-J  & ROUGE   & BGE  & LLM-A-J  \\ \hline
% Initial       &        &      &          &         &      &          \\
% Random        &        &      &          &         &      &          \\
% SelectIT      &        &      &          &         &      &          \\
% LESS          &        &      &          &         &      &          \\
% SE Feat. &        &      &          &         &      &          \\
% Util. Feat.      &        &      &          &         &      &          \\
% Full Data     &        &      &          &         &      &          \\ \hline
% \end{tabular}
% \caption{Results on Qwen2 on MixInstruct and MT-Bench ("LLM-A-J" refers to LLM-As-Judges)}
% \label{uc2: qwen-mix-mtbench}
% \end{table}

\begin{table}[]
\centering\small
\makebox[\linewidth][c]{%
\begin{tabular}{lcccccccccccc}
\toprule
\multicolumn{1}{l}{Model} & \multicolumn{6}{c}{Qwen2}                                                                                              & \multicolumn{6}{c}{Phi-3}                                                                                             \\ \cmidrule(lr){2-7} \cmidrule(lr){8-13}
Method                     & \multicolumn{3}{c}{ICL}                                                    & \multicolumn{3}{c}{QLoRA}                      & \multicolumn{3}{c}{ICL}                                                                & \multicolumn{3}{c}{QLoRA}                             \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
                           & ROUGE                & BGE            & \multicolumn{1}{c}{LAJ}           & ROUGE          & BGE            & LAJ           & ROUGE                & BGE                  & \multicolumn{1}{c}{LAJ}                 & ROUGE          & BGE                  & LAJ           \\ \midrule
Initial                    &                 &                 & \multicolumn{1}{c}{}                &           &                 &           &                 &                 & \multicolumn{1}{c}{}                &           &                 &           \\
Random                     &                 &                 & \multicolumn{1}{c}{}                &           &                 &           &                 &                 & \multicolumn{1}{c}{}                &           &                 &           \\
SelectIT                   &                 &                 & \multicolumn{1}{c}{}                &           &                 &           &                 &                 & \multicolumn{1}{c}{}                &           &                 &           \\
LESS                       &                 &                 & \multicolumn{1}{c}{}                &           &                 &           &                 & {\ul }          & \multicolumn{1}{c}{}                &           & {\ul }          &           \\
SE Feat.                   &                 &                 & \multicolumn{1}{c}{}                &           &                 &           &                 &                 & \multicolumn{1}{c}{}                &           &                 &           \\
Util. Feat.                & {\ul \textbf{}} & {\ul \textbf{}} & \multicolumn{1}{c}{{\ul \textbf{}}} & {\ul }    & {\ul \textbf{}} & {\ul }    & {\ul \textbf{}} & {\ul \textbf{}} & \multicolumn{1}{c}{{\ul \textbf{}}} & {\ul }    & {\ul \textbf{}} & {\ul }    \\
Full Data                  & {\ul \textbf{}} & {\ul \textbf{}} & \multicolumn{1}{c}{{\ul \textbf{}}} & \textbf{} & {\ul \textbf{}} & \textbf{} & {\ul \textbf{}} & {\ul \textbf{}} & \multicolumn{1}{c}{{\ul \textbf{}}} & \textbf{} & {\ul \textbf{}} & \textbf{} \\ \bottomrule
\end{tabular}
}
\caption{Results on Use Case 2: MixInstruct and MT-Bench ("LAJ" refers to LLM-As-Judges). \textbf{Bold} and {\ul underline} indicate best and second-best performance, respectively.}
\label{uc2: qwen-phi-mi-mtbench}
\end{table}

\begin{table}[]
\centering\small
\makebox[\linewidth][c]{%
\begin{tabular}{lcc}
\toprule
\multicolumn{1}{l}{Model} & \multicolumn{1}{c}{Qwen2} & \multicolumn{1}{c}{Phi-3} \\ \midrule
Method                     & QLoRA                          & QLoRA                          \\ \midrule
Initial                    & 82.10                          & 69.10                          \\
Random                     & 79.31                          & 65.16                          \\
SelectIT                   & 79.13                          & 65.24                          \\
LESS                       & {\ul 80.35}                    & {\ul 66.72}                    \\
SE Feat.                   & 80.10                          & 66.36                          \\
Util. Feat.                & \textbf{81.70}                 & \textbf{68.70}                 \\
Full Data                  & 78.36                          & 64.50                          \\ \bottomrule
\end{tabular}
}
\caption{Classification Accuracy on Use Case 2: HotpotQA and MMLU. We report the MMLU test accuracy in a 5 shot setting. There is a 5.51\% performance percentage \textit{improvement} from Full Data to Util. Feat. after pruning 70\% of the data, and a 2.29\% performance percentage drop from Util. Feat. to the next best baseline.}%Results show that by fine-tuning on HotpotQA, there is a drastic performance degradation of MMLU performance using the full data. However, the performance degradation is minimized when training on subsets selected by \sysn{}.}
\label{uc2: qwen-phi-hotpot-mmlu}
\end{table}




==> tables/continual_learning.tex <==
% \begin{table}[]
% \centering
% \begin{tabular}{c|ccc|ccc}
% \hline
% Method        & \multicolumn{3}{c|}{ICL}                        & \multicolumn{3}{c}{QLoRA}                       \\ \hline
%               & ROUGE          & BGE            & LLM-A-J       & ROUGE          & BGE            & LLM-A-J       \\ \hline
% Initial       & 44.11          & 70.49          & 2.43          & 48.49          & 80.85          & 2.62          \\
% Random        & 55.57          & 85.26          & 2.91          & 55.52          & 85.53          & 2.94          \\
% SelectIT      & 63.07          & 86.38          & 3.18          & 65.42          & 87.50          & 3.20          \\
% LESS          & 64.28          & 85.41          & 3.29          & 69.85          & 89.33          & 3.45          \\
% SE Feat. & 61.07          & 85.16          & 3.45          & 74.05          & 92.47          & 3.58          \\
% Util. Feat.      & \textbf{69.49} & \textbf{87.94} & {\ul 3.60}    & {\ul 74.19}    & {\ul 92.23}    & {\ul 3.65}    \\
% Full Data     & {\ul 66.08}    & {\ul 87.84}    & \textbf{3.65} & \textbf{76.83} & \textbf{92.63} & \textbf{3.74} \\ \hline
% \end{tabular}
% \caption{Results on Qwen2 on IBM and Government ("LLM-A-J" refers to LLM-As-Judges)}
% \label{uc3: qwen-ibm-gov}
% \end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{c|ccc|ccc}
% \hline
% Method        & \multicolumn{3}{c|}{ICL} & \multicolumn{3}{c}{QLoRA} \\ \hline
%               & ROUGE  & BGE  & LLM-A-J  & ROUGE   & BGE  & LLM-A-J  \\ \hline
% Initial       & 40.66          & 58.68          & 1.52          & 43.96          & 69.56          & 2.29          \\
% Random        & 45.76          & 76.19          & 2.45          & 58.94          & 82.41          & 2.89          \\
% SelectIT      & 63.49          & 85.27          & 2.96          & 64.09          & 85.07          & 3.16          \\
% LESS          & 66.01          & 87.20          & 3.19          & 67.53          & 88.17          & 3.22          \\
% SE Feat. & 68.84          & 88.46          & 3.32          & 69.30          & 88.62          & 3.35          \\
% Util. Feat.      & \textbf{74.11} & {\ul 89.41}    & \textbf{3.57} & {\ul 74.38}    & \textbf{91.55} & {\ul 3.57}    \\
% Full Data     & {\ul 71.23}    & \textbf{91.10} & {\ul 3.52}    & \textbf{77.12} & {\ul 91.10}    & \textbf{3.64} \\ \hline
% \end{tabular}
% \caption{Results on Phi-3 on IBM and Government ("LLM-A-J" refers to LLM-As-Judges)}
% \label{uc3: phi-ibm-gov}
% \end{table}

\begin{table}[]
\centering\small
\makebox[\linewidth][c]{%
\begin{tabular}{lcccccccccccc}
\toprule
\multicolumn{1}{l}{Model} & \multicolumn{6}{c}{Qwen2}                                                                                              & \multicolumn{6}{c}{Phi-3}                                                                                             \\ \cmidrule(lr){2-7} \cmidrule(lr){8-13}
Method                     & \multicolumn{3}{c}{ICL}                                                    & \multicolumn{3}{c}{QLoRA}                      & \multicolumn{3}{c}{ICL}                                                                & \multicolumn{3}{c}{QLoRA}                             \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
                           & ROUGE                & BGE            & \multicolumn{1}{c}{LAJ}           & ROUGE          & BGE            & LAJ           & ROUGE                & BGE                  & \multicolumn{1}{c}{LAJ}                 & ROUGE          & BGE                  & LAJ           \\ \midrule
Initial     & 44.11          & 70.49          & \multicolumn{1}{c}{2.43}          & 48.49          & 80.85          & 2.62          & 40.66          & 58.68          & \multicolumn{1}{c}{1.52}          & 43.96          & 69.56          & 2.29          \\
Random      & 55.57          & 85.26          & \multicolumn{1}{c}{2.91}          & 55.52          & 85.53          & 2.94          & 45.76          & 76.19          & \multicolumn{1}{c}{2.45}          & 58.94          & 82.41          & 2.89          \\
SelectIT    & 63.07          & 86.38          & \multicolumn{1}{c}{3.18}          & 65.42          & 87.50          & 3.20          & 63.49          & 85.27          & \multicolumn{1}{c}{2.96}          & 64.09          & 85.07          & 3.16          \\
LESS        & 64.28          & 85.41          & \multicolumn{1}{c}{3.29}          & 69.85          & 89.33          & 3.45          & 66.01          & 87.20          & \multicolumn{1}{c}{3.19}          & 67.53          & 88.17          & 3.22          \\
SE Feat.    & 61.07          & 85.16          & \multicolumn{1}{c}{3.45}          & 74.05          & 92.47          & 3.58          & 68.84          & 88.46          & \multicolumn{1}{c}{3.32}          & 69.30          & 88.62          & 3.35          \\
Util. Feat. & \textbf{69.49} & \textbf{87.94} & \multicolumn{1}{c}{{\ul 3.60}}    & {\ul 74.19}    & {\ul 92.23}    & {\ul 3.65}    & \textbf{74.11} & {\ul 89.41}    & \multicolumn{1}{c}{\textbf{3.57}} & {\ul 74.38}    & \textbf{91.55} & {\ul 3.57}    \\
Full Data   & {\ul 66.08}    & {\ul 87.84}    & \multicolumn{1}{c}{\textbf{3.65}} & \textbf{76.83} & \textbf{92.63} & \textbf{3.74} & {\ul 71.23}    & \textbf{91.10} & \multicolumn{1}{c}{{\ul 3.52}}    & \textbf{77.12} & {\ul 91.10}    & \textbf{3.64} \\ \bottomrule


\end{tabular}
}
\caption{Results on Use Case 3: IBM and Government. \textbf{Bold} and {\ul underline} indicate best and second-best performance, respectively. There is \textit{only} a 0.31\% performance percentage drop from Full Data to Util. Feat. after pruning 70\% of the data, and a 3.89\% performance percentage drop from Util. Feat. to the next best baseline.}
\label{uc3: qwen-phi-ibm-gov}
\end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{c|ccc|ccc}
% \hline
% Method        & \multicolumn{3}{c|}{ICL}                        & \multicolumn{3}{c}{QLoRA}                       \\ \hline
%               & ROUGE          & BGE            & LLM-A-J       & ROUGE          & BGE            & LLM-A-J       \\ \hline
% Initial       & 51.51          & 66.97          & 1.77          & 54.18          & 78.27          & 2.5           \\
% Random        & 54.38          & 79.12          & 2.57          & 59.23          & 82.02          & 2.66          \\
% SelectIT      & 58.03          & 83.75          & 2.82          & 63.26          & 84.01          & 2.87          \\
% LESS          & 67.16          & 85.76          & 2.94          & 69.72          & 86.63          & 3.26          \\
% SE Feat. & 73.75          & 88.01          & 3.26          & 74.84          & 88.79          & 3.30          \\
% Util. Feat.      & {\ul 76.94}    & \textbf{90.41} & {\ul 3.33}    & {\ul 77.56}    & {\ul 89.99}    & {\ul 3.34}    \\
% Full Data     & \textbf{77.78} & {\ul 90.31}    & \textbf{3.35} & \textbf{78.72} & \textbf{90.77} & \textbf{3.48} \\ \hline
% \end{tabular}
% \caption{Results on Qwen2 on SQuAD and HotpotQA ("LLM-A-J" refers to LLM-As-Judges)}
% \label{uc3: qwen-squad-hotpot}
% \end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{c|ccc|ccc}
% \hline
% Method        & \multicolumn{3}{c|}{ICL}                        & \multicolumn{3}{c}{QLoRA}                       \\ \hline
%               & ROUGE          & BGE            & LLM-A-J       & ROUGE          & BGE            & LLM-A-J       \\ \hline
% Initial       & 40.42          & 58.23          & 1.26          & 40.94          & 58.12          & 1.29          \\
% Random        & 44.29          & 59.45          & 1.33          & 50.29          & 61.52          & 1.60          \\
% SelectIT      & 47.35          & 74.15          & 2.54          & 56.88          & 80.47          & 2.70          \\
% LESS          & 60.97          & 81.41          & 2.84          & 61.56          & 81.53          & 2.88          \\
% SE Feat. & 64.44          & 83.95          & 3.03          & 66.35          & 84.77          & 3.14          \\
% Util. Feat.      & {\ul 66.55}    & {\ul 84.65}    & {\ul 3.25}    & {\ul 67.09}    & {\ul 85.17}    & {\ul 3.32}    \\
% Full Data     & \textbf{68.47} & \textbf{85.93} & \textbf{3.33} & \textbf{70.48} & \textbf{86.06} & \textbf{3.44} \\ \hline
% \end{tabular}
% \caption{Results on Phi-3 on SQuAD and HotpotQA ("LLM-A-J" refers to LLM-As-Judges)}
% \label{uc3: phi-squad-hotpot}
% \end{table}

\begin{table}[]
\centering\small
\makebox[\linewidth][c]{%
\begin{tabular}{lcccccccccccc}
\toprule
\multicolumn{1}{l}{Model} & \multicolumn{6}{c}{Qwen2}                                                                                              & \multicolumn{6}{c}{Phi-3}                                                                                             \\ \cmidrule(lr){2-7} \cmidrule(lr){8-13}
Method                     & \multicolumn{3}{c}{ICL}                                                    & \multicolumn{3}{c}{QLoRA}                      & \multicolumn{3}{c}{ICL}                                                                & \multicolumn{3}{c}{QLoRA}                             \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
                           & ROUGE                & BGE            & \multicolumn{1}{c}{LAJ}           & ROUGE          & BGE            & LAJ           & ROUGE                & BGE                  & \multicolumn{1}{c}{LAJ}             & ROUGE          & BGE                  & LAJ       \\ \midrule
Initial     & 51.51          & 66.97          & \multicolumn{1}{c}{1.77}          & 54.18          & 78.27          & 2.50          & 40.42          & 58.23          & \multicolumn{1}{c}{1.26}          & 40.94          & 58.12          & 1.29          \\
Random      & 54.38          & 79.12          & \multicolumn{1}{c}{2.57}          & 59.23          & 82.02          & 2.66          & 44.29          & 59.45          & \multicolumn{1}{c}{1.33}          & 50.29          & 61.52          & 1.60          \\
SelectIT    & 58.03          & 83.75          & \multicolumn{1}{c}{2.82}          & 63.26          & 84.01          & 2.87          & 47.35          & 74.15          & \multicolumn{1}{c}{2.54}          & 56.88          & 80.47          & 2.70          \\
LESS        & 67.16          & 85.76          & \multicolumn{1}{c}{2.94}          & 69.72          & 86.63          & 3.26          & 60.97          & 81.41          & \multicolumn{1}{c}{2.84}          & 61.56          & 81.53          & 2.88          \\
SE Feat.    & 73.75          & 88.01          & \multicolumn{1}{c}{3.26}          & 74.84          & 88.79          & 3.30          & 64.44          & 83.95          & \multicolumn{1}{c}{3.03}          & 66.35          & 84.77          & 3.14          \\
Util. Feat. & {\ul 76.94}    & \textbf{90.41} & \multicolumn{1}{c}{{\ul 3.33}}    & {\ul 77.56}    & {\ul 89.99}    & {\ul 3.34}    & {\ul 66.55}    & {\ul 84.65}    & \multicolumn{1}{c}{{\ul 3.25}}    & {\ul 67.09}    & {\ul 85.17}    & {\ul 3.32}    \\
Full Data   & \textbf{77.78} & {\ul 90.31}    & \multicolumn{1}{c}{\textbf{3.35}} & \textbf{78.72} & \textbf{90.77} & \textbf{3.48} & \textbf{68.47} & \textbf{85.93} & \multicolumn{1}{c}{\textbf{3.33}} & \textbf{70.48} & \textbf{86.06} & \textbf{3.44} \\ \bottomrule


\end{tabular}
}
\caption{Results on Use Case 3: SQuAD and HotpotQA.  \textbf{Bold} and {\ul underline} indicate best and second-best performance, respectively. There is \textit{only} a 1.94\% performance percentage drop from Full Data to Util. Feat. after pruning 70\% of the data, and a 2.78\% performance percentage drop from Util. Feat. to the next best baseline.}
\label{uc3: qwen-phi-squad-hotpot}
\end{table}

\begin{table}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccc|cccccc}
\toprule
\multicolumn{1}{l}{Model} & \multicolumn{6}{c|}{Qwen2} & \multicolumn{6}{c}{Phi-3} \\ \cmidrule(lr){2-7} \cmidrule(lr){8-13}
                          & \multicolumn{3}{c}{ICL} & \multicolumn{3}{c|}{QLoRA} & \multicolumn{3}{c}{ICL} & \multicolumn{3}{c}{QLoRA} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
                          & ROUGE & BGE  & LAJ  & ROUGE & BGE  & LAJ  & ROUGE & BGE   & LAJ  & ROUGE & BGE   & LAJ  \\ \midrule
Initial                   & 51.51 & 66.97 & 1.77 & 54.18 & 78.27 & 2.50 & 40.42 & 58.23 & 1.26 & 40.94 & 58.12 & 1.29 \\
Random                    & 54.38 & 79.12 & 2.57 & 59.23 & 82.02 & 2.66 & 44.29 & 59.45 & 1.33 & 50.29 & 61.52 & 1.60 \\
SelectIT                  & 58.03 & 83.75 & 2.82 & 63.26 & 84.01 & 2.87 & 47.35 & 74.15 & 2.54 & 56.88 & 80.47 & 2.70 \\
LESS                      & 67.16 & 85.76 & 2.94 & 69.72 & 86.63 & 3.26 & 60.97 & 81.41 & 2.84 & 61.56 & 81.53 & 2.88 \\
SE Feat.                  & 73.75 & 88.01 & 3.26 & 74.84 & 88.79 & 3.30 & 64.44 & 83.95 & 3.03 & 66.35 & 84.77 & 3.14 \\
Util. Feat.               & {\ul 76.94} & \textbf{90.41} & {\ul 3.33} & {\ul 77.56} & {\ul 89.99} & {\ul 3.34} & {\ul 66.55} & {\ul 84.65} & {\ul 3.25} & {\ul 67.09} & {\ul 85.17} & {\ul 3.32} \\
Full Data                 & \textbf{77.78} & {\ul 90.31} & \textbf{3.35} & \textbf{78.72} & \textbf{90.77} & \textbf{3.48} & \textbf{68.47} & \textbf{85.93} & \textbf{3.33} & \textbf{70.48} & \textbf{86.06} & \textbf{3.44} \\ \bottomrule
\end{tabular}%
}
\caption{Results on Use Case 3: SQuAD and HotpotQA. \textbf{Bold} and {\ul underline} indicate best and second-best performance, respectively. There is \textit{only} a 1.94\% performance percentage drop from Full Data to Util. Feat. after pruning 70\% of the data, and a 2.78\% performance percentage drop from Util. Feat. to the next best baseline.}
\label{uc3: qwen-phi-squad-hotpot}
\end{table}


==> tables/distributions.tex <==
\begin{table}[]
\centering
\label{llmaj_score_dist_1}
\caption{LLM-as-Judges score distributions for Use Case 1 with MixInstruct training and validation set on the Qwen2-72B-Instruct model on the Initial, Random, and SelectIT baselines. The corresponding table is Table \ref{uc1: qwen-mi-mi}.}
\begin{tabular}{c|cc}
\hline
\multicolumn{1}{c|}{} & ICL & QLoRA \\ \hline
Initial               & \includegraphics[scale=0.3]{llmaj_score_distributions/initial-ICL.pdf}    & \includegraphics[scale=0.3]{llmaj_score_distributions/initial-PEFT.pdf}      \\
Random                & \includegraphics[scale=0.3]{llmaj_score_distributions/random-ICL.pdf}    & \includegraphics[scale=0.3]{llmaj_score_distributions/random-PEFT.pdf}      \\
SelectIT              & \includegraphics[scale=0.3]{llmaj_score_distributions/select_it-ICL.pdf}    & \includegraphics[scale=0.3]{llmaj_score_distributions/select_it-PEFT.pdf}      \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\centering
\label{score_distribution_pt2}
\caption{LLM-as-Judges score distributions for Use Case 1 with MixInstruct training and validation set on the Qwen2-72B-Instruct model on the LESS, Semantic Similarity Utility, and Full Data baselines, and our ICL Utility. The corresponding table is Table \ref{uc1: qwen-mi-mi}.}
\begin{tabular}{c|cc}
\hline
\multicolumn{1}{c|}{} & ICL & QLoRA \\ \hline
LESS                  & \includegraphics[scale=0.3]{llmaj_score_distributions/less-ICL.pdf}    & \includegraphics[scale=0.3]{llmaj_score_distributions/less-PEFT.pdf}      \\
Sem Sim Util.         & \includegraphics[scale=0.3]{llmaj_score_distributions/mod_ind_fl-ICL.pdf}    & \includegraphics[scale=0.3]{llmaj_score_distributions/mod_ind_fl-PEFT.pdf}      \\
ICL Util              & \includegraphics[scale=0.3]{llmaj_score_distributions/mod_dep_fl-ICL.pdf}    &  \includegraphics[scale=0.3]{llmaj_score_distributions/mod_dep_fl-PEFT.pdf}     \\
Full Data             & \includegraphics[scale=0.3]{llmaj_score_distributions/full_data-ICL.pdf}    &  \includegraphics[scale=0.3]{llmaj_score_distributions/full_data-PEFT.pdf}     \\ \hline
\end{tabular}
\end{table}

==> tables/same_dataset.tex <==
% \begin{table}[]
% \centering
% \begin{tabular}{c|ccc|ccc}
% \hline
% Method        & \multicolumn{3}{c|}{ICL}                        & \multicolumn{3}{c}{QLoRA}                       \\ \hline
%               & ROUGE          & BGE            & LLM-A-J       & ROUGE          & BGE            & LLM-A-J       \\ \hline
% Initial       & 37.87          & 78.92          & 2.98          & 36.36          & 82.55          & 3.02          \\
% Random        & 39.00          & 80.66          & 3.12          & 44.45          & 85.46          & 3.12          \\
% SelectIT      & 43.08          & 84.50          & 3.18          & 45.14          & 85.88          & 3.21          \\
% LESS          & 42.08          & 83.24          & 3.26          & 45.16          & 84.95          & 3.28          \\
% SE Feat. & 47.43          & 84.40          & 3.28          & 48.22          & 86.50          & 3.28          \\
% Util. Feat.      & {\ul 48.46}    & {\ul 85.77}    & {\ul 3.35}    & {\ul 52.79}    & {\ul 88.04}    & {\ul 3.37}    \\
% Full Data     & \textbf{58.65} & \textbf{88.72} & \textbf{3.45} & \textbf{65.51} & \textbf{92.24} & \textbf{3.51} \\ \hline
% \end{tabular}
% \caption{Results on Qwen2 on MixInstruct ("LLM-A-J" refers to LLM-As-Judges).}
% \label{uc1: qwen-mi-mi}
% \end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{c|ccc|ccc}
% \hline
% Method        & \multicolumn{3}{c|}{ICL}                        & \multicolumn{3}{c}{QLoRA}                       \\ \hline
%               & ROUGE          & BGE            & LLM-A-J       & ROUGE          & BGE            & LLM-A-J       \\ \hline
% Initial       & 25.76          & 43.34          & 1.42          & 35.50          & 80.46          & 2.58          \\
% Random        & 33.05          & 72.73          & 2.92          & 44.70          & 83.75          & 2.95          \\
% SelectIT      & 36.11          & 76.31          & 3.18          & 49.68          & 85.84          & 3.20          \\
% LESS          & 47.10          & {\ul 85.94}    & 3.23          & 48.68          & {\ul 85.86}    & 3.24          \\
% SE Feat. & 46.62          & 85.28          & 3.24          & 45.64          & 83.70          & 3.27          \\
% Util. Feat.      & {\ul 49.83}    & 85.27          & {\ul 3.32}    & {\ul 50.31}    & 84.40          & {\ul 3.33}    \\
% Full Data     & \textbf{55.92} & \textbf{88.26} & \textbf{3.45} & \textbf{74.98} & \textbf{93.33} & \textbf{3.84} \\ \hline
% \end{tabular}
% \caption{Results on Phi-3 on MixInstruct ("LLM-A-J" refers to LLM-As-Judges).}
% \label{uc1: phi-mi-mi}
% \end{table}

\begin{table}[]
\centering\small
\makebox[\linewidth][c]{%
\begin{tabular}{lcccccccccccc}
\toprule
\multicolumn{1}{l}{Model} & \multicolumn{6}{c}{Qwen2}                                                                                              & \multicolumn{6}{c}{Phi-3}                                                                                             \\ \cmidrule(lr){2-7} \cmidrule(lr){8-13}
Method                     & \multicolumn{3}{c}{ICL}                                                    & \multicolumn{3}{c}{QLoRA}                      & \multicolumn{3}{c}{ICL}                                                                & \multicolumn{3}{c}{QLoRA}                             \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
                           & ROUGE                & BGE            & \multicolumn{1}{c}{LAJ}           & ROUGE          & BGE            & LAJ           & ROUGE                & BGE                  & \multicolumn{1}{c}{LAJ}                 & ROUGE          & BGE                  & LAJ           \\ \midrule
Initial     & 37.87          & 78.92          & \multicolumn{1}{c}{2.98}          & 36.36          & 82.55          & 3.02          & 25.76          & 43.34          & \multicolumn{1}{c}{1.42}          & 35.50          & 80.46          & 2.58          \\
Random      & 39.00          & 80.66          & \multicolumn{1}{c}{3.12}          & 44.45          & 85.46          & 3.12          & 33.05          & 72.73          & \multicolumn{1}{c}{2.92}          & 44.70          & 83.75          & 2.95          \\
SelectIT    & 43.08          & 84.50          & \multicolumn{1}{c}{3.18}          & 45.14          & 85.88          & 3.21          & 36.11          & 76.31          & \multicolumn{1}{c}{3.18}          & 49.68          & 85.84          & 3.20          \\
LESS        & 42.08          & 83.24          & \multicolumn{1}{c}{3.26}          & 45.16          & 84.95          & 3.28          & 47.10          & \textbf{85.94} & \multicolumn{1}{c}{3.23}          & 48.68          & {\ul 85.86}    & 3.24          \\
SE Feat.    & 47.43          & 84.40          & \multicolumn{1}{c}{3.28}          & 48.22          & 86.50          & 3.28          & 46.62          & 85.28          & \multicolumn{1}{c}{3.24}          & 45.64          & 83.70          & 3.27          \\
Util. Feat. & {\ul 48.46}    & {\ul 85.77}    & \multicolumn{1}{c}{{\ul 3.35}}    & {\ul 52.79}    & {\ul 88.04}    & {\ul 3.37}    & {\ul 49.83}    & 85.27          & \multicolumn{1}{c}{{\ul 3.32}}    & {\ul 50.31}    & 84.40          & {\ul 3.33}    \\
Full Data   & \textbf{58.65} & \textbf{88.72} & \multicolumn{1}{c}{\textbf{3.45}} & \textbf{65.51} & \textbf{92.24} & \textbf{3.51} & \textbf{55.92} & {\ul 88.26}    & \multicolumn{1}{c}{\textbf{3.45}} & \textbf{74.98} & \textbf{93.33} & \textbf{3.84} \\ \bottomrule

\end{tabular}
}
\caption{Results on Use Case 1: MixInstruct. \textbf{Bold} and {\ul underline} indicate best and second-best performance, respectively. There is a 10.44\% performance percentage drop from Full Data to Util. Feat. after pruning 70\% of the data, and a 2.27\% performance percentage drop from Util. Feat. to the next best baseline.}
\label{uc1: qwen-phi-mix-instruct}
\end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{c|ccc|ccc}
% \hline
% Method        & \multicolumn{3}{c|}{ICL}                        & \multicolumn{3}{c}{QLoRA}                       \\ \hline
%               & ROUGE          & BGE            & LLM-A-J       & ROUGE          & BGE            & LLM-A-J       \\ \hline
% Initial       & 18.03          & 59.13          & 1.54          & 20.15          & 58.38          & 1.78          \\
% Random        & 20.05          & 59.39          & 1.79          & 20.29          & 59.39          & 1.83          \\
% SelectIT      & 31.38          & 71.08          & 2.86          & 32.96          & 74.76          & 2.90          \\
% LESS          & 34.59          & 83.23          & 3.07          & 35.03          & 83.37          & 3.50          \\
% SE Feat. & 34.69          & 83.31          & 3.43          & 35.46          & 83.43          & 3.53          \\
% Util. Feat.      & {\ul 35.48}    & {\ul 83.69}    & \textbf{3.58}    & {\ul 35.60}    & \textbf{83.64}    & {\ul 3.54}    \\
% Full Data     & \textbf{36.43} & \textbf{84.25} & {\ul 3.53} & \textbf{35.88} & {\ul 76.87} & \textbf{3.63} \\ \hline
% \end{tabular}
% \caption{Results on Qwen2 on P3 ("LLM-A-J" refers to LLM-As-Judges)}
% \label{uc1: qwen-p3-p3}
% \end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{c|ccc|ccc}
% \hline
% Method        & \multicolumn{3}{c|}{ICL}                        & \multicolumn{3}{c}{QLoRA}                       \\ \hline
%               & ROUGE          & BGE            & LLM-A-J       & ROUGE          & BGE            & LLM-A-J       \\ \hline
% Initial       & 20.10          & 48.66          & 1.36          & 20.64          & 49.17          & 1.39          \\
% Random        & 20.83          & 49.92          & 2.24          & 24.51          & 53.41          & 2.36          \\
% SelectIT      & 35.37          & 66.67          & 2.52          & 38.98          & 69.84          & 2.54          \\
% LESS          & 39.69          & 72.12          & 3.17          & 40.32          & 70.89          & 3.24          \\
% SE Feat. & 37.07          & 71.49          & 3.52          & 38.13          & 79.68          & 3.74          \\
% Util. Feat.      & {\ul 40.66}    & {\ul 84.00}    & {\ul 3.68}    & {\ul 41.91}    & {\ul 84.53}    & {\ul 3.76}    \\
% Full Data     & \textbf{42.07} & \textbf{85.26} & \textbf{3.78} & \textbf{44.73} & \textbf{87.03} & \textbf{3.82} \\ \hline
% \end{tabular}
% \caption{Results on Phi-3 on P3 ("LLM-A-J" refers to LLM-As-Judges)}
% \label{uc1: phi-p3-p3}
% \end{table}

\begin{table}[]
\centering\small
\makebox[\linewidth][c]{%
\begin{tabular}{lcccccccccccc}
\toprule
\multicolumn{1}{l}{Model} & \multicolumn{6}{c}{Qwen2}                                                                                              & \multicolumn{6}{c}{Phi-3}                                                                                             \\ \cmidrule(lr){2-7} \cmidrule(lr){8-13}
Method                     & \multicolumn{3}{c}{ICL}                                                    & \multicolumn{3}{c}{QLoRA}                      & \multicolumn{3}{c}{ICL}                                                                & \multicolumn{3}{c}{QLoRA}                             \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
                           & ROUGE                & BGE            & \multicolumn{1}{c}{LAJ}           & ROUGE          & BGE            & LAJ           & ROUGE                & BGE                  & \multicolumn{1}{c}{LAJ}                 & ROUGE          & BGE                  & LAJ           \\ \midrule
Initial     & 18.03          & 59.13          & \multicolumn{1}{c}{1.54}          & 20.15          & 58.38          & 1.78          & 20.10          & 48.66          & \multicolumn{1}{c}{1.36}          & 20.64          & 49.17          & 1.39          \\
Random      & 20.05          & 59.39          & \multicolumn{1}{c}{1.79}          & 20.29          & 59.39          & 1.83          & 20.83          & 49.92          & \multicolumn{1}{c}{2.24}          & 24.51          & 53.41          & 2.36          \\
SelectIT    & 31.38          & 71.08          & \multicolumn{1}{c}{2.86}          & 32.96          & 74.76          & 2.90          & 35.37          & 66.67          & \multicolumn{1}{c}{2.52}          & 38.98          & 69.84          & 2.54          \\
LESS        & 34.59          & 83.23          & \multicolumn{1}{c}{3.07}          & 35.03          & 83.37          & 3.50          & 39.69          & 72.12          & \multicolumn{1}{c}{3.17}          & 40.32          & 70.89          & 3.24          \\
SE Feat.    & 34.69          & 83.31          & \multicolumn{1}{c}{3.43}          & 35.46          & {\ul 83.43}    & 3.53          & 37.07          & 71.49          & \multicolumn{1}{c}{3.52}          & 38.13          & 79.68          & 3.74          \\
Util. Feat. & {\ul 35.48}    & {\ul 83.69}    & \multicolumn{1}{c}{\textbf{3.58}} & {\ul 35.60}    & \textbf{83.64} & {\ul 3.54}    & {\ul 40.66}    & {\ul 84.00}    & \multicolumn{1}{c}{{\ul 3.68}}    & {\ul 41.91}    & {\ul 84.53}    & {\ul 3.76}    \\
Full Data   & \textbf{36.43} & \textbf{84.25} & \multicolumn{1}{c}{{\ul 3.53}}    & \textbf{35.88} & 76.87          & \textbf{3.63} & \textbf{42.07} & \textbf{85.26} & \multicolumn{1}{c}{\textbf{3.78}} & \textbf{44.73} & \textbf{87.03} & \textbf{3.82} \\ \bottomrule

\end{tabular}
}
\caption{Results on Use Case 1: P3. \textbf{Bold} and {\ul underline} indicate best and second-best performance, respectively. There is \textit{only} a 0.76\% performance percentage drop from Full Data to Util. Feat. after pruning 70\% of the data, and a 3.23\% performance percentage drop from Util. Feat. to the next best baseline.}
\label{uc1: qwen-phi-p3}
\end{table}
